Nonlinear Dynamics of Coupled-Resonator Kerr-Combs

The nonlinear interaction of a microresonator pumped by a laser has revealed complex dynamics including soliton formation and chaos. Initial studies of coupled-resonator systems reveal even more complicated dynamics that can lead to deterministic modelocking and efficient comb generation. Here we perform theoretical analysis and experiments that provide insight into the dynamical behavior of coupled-resonator systems operating in the normal group-velocity-dispersion regime. Our stability analysis and simulations reveal that the strong mode-coupling regime, which gives rise to spectrally-broad comb states, can lead to an instability mechanism in the auxiliary resonator that destabilizes the comb state and prevents mode-locking. We find that this instability can be suppressed by introducing loss in the auxiliary resonator. We investigate the stability of both single- and multi-pulse solutions and verify our theoretical predictions by performing experiments in a silicon-nitride platform. Our results provide an understanding for accessing broad, efficient, relatively flat high-power mode-locked combs for numerous applications in spectroscopy, time-frequency metrology, and data communications.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
